Pure Exploration and Regret Minimization in Matching Bandits

Finding an optimal matching in a weighted graph is a standard combinatorial problem. We consider its semi-bandit version where either a pair or a full matching is sampled sequentially. We prove that it is possible to leverage a rank-1 assumption on the adjacency matrix to reduce the sample complexity and the regret of off-the-shelf algorithms up to reaching a linear dependency in the number of vertices (up to poly log terms).

==> Learning Matchings/prelude.tex <==
\usepackage{microtype}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{thmtools}
\usepackage{thm-restate}
%\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$\textit{#1}}

\usepackage{geometry}
\geometry{margin=0.8in}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\usepackage{hyperref}

\usepackage{breakcites}
\newcommand{\theHalgorithm}{\arabic{algorithm}}


\usepackage[utf8]{inputenc}

\usepackage{amsmath,amsfonts,hyperref}
%\usepackage[table,xcdraw]{xcolor}
\usepackage{dsfont}
%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{array,multirow,graphicx}
\usepackage{float}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{caption}
%\usepackage{subcaption}

%\usepackage{mathpazo}

\usepackage{comment}

\usepackage{slantsc}
\setlength{\parskip}{0.3em}

\DeclareMathOperator*{\argmax}{arg\,max} 

\makeatletter
\newenvironment{algosketch}[1][htb]{%
    \renewcommand{\ALG@name}{Algorithm Sketch}% Update algorithm name
   \begin{algorithm}[#1]%
  }{\end{algorithm}}
\makeatother

\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\declaretheorem[name=Theorem,numberwithin=section]{thm}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{hyp}{Assumption}

\newcommand{\V}{\mathcal{V}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\usepackage{algorithm}
\usepackage{algorithmic}

\newcommand{\SRankElim}{{\sc Pair-Elim}}
\newcommand{\RankElim}{{\sc Rank1Elim}}
\newcommand{\IBLearning}{{\sc Pair-Select}}
\newcommand{\IBLearningname}{Pair Select}
\newcommand{\RMono}{{\sc Pair-Elim-Mono}}
\newcommand{\SMDC}{{\sc simple-Adaptive-Matching}}
\newcommand{\SMDCname}{Simple Adaptive Matching}
\newcommand{\MatchingId}{{\sc Matching-id}}
%\newcommand{\SMDCname}{Simplified Matching Divide and Conquer algorithm}
\newcommand{\MDC}{{\sc Adaptive-Matching}}
\newcommand{\MDCname}{Adaptive Matching}
%\newcommand{\MDCname}{Matching Divide and Conquer}
\newcommand{\CMSampling}{{\sc Sample-Matching}}
\newcommand{\SEBElim}{{\sc Row-Col-Elim}}
\newcommand{\SEBElimR}{{\sc Row-Elim}}
\newcommand{\SEBElimC}{{\sc Col-Elim}}

\newcommand{\fs}[1]{\textcolor{red}{#1}}
\newcommand{\mv}[1]{\textcolor{blue}{#1}}
\newcommand{\jy}[1]{\textcolor{cyan}{#1}}
\newcommand{\cc}[1]{\textcolor{red}{#1}}
\newcommand{\vp}[1]{\textcolor{magenta}{#1}}

\author{%
 
}

==> prelude.tex <==
\usepackage{microtype}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{thmtools}
\usepackage{thm-restate}
%\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$\textit{#1}}

\usepackage{geometry}
\geometry{margin=0.8in}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\usepackage{hyperref}

\usepackage{breakcites}
\newcommand{\theHalgorithm}{\arabic{algorithm}}


\usepackage[utf8]{inputenc}

\usepackage{amsmath,amsfonts,hyperref}
%\usepackage[table,xcdraw]{xcolor}
\usepackage{dsfont}
%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{array,multirow,graphicx}
\usepackage{float}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{caption}
%\usepackage{subcaption}

%\usepackage{mathpazo}

\usepackage{comment}

\usepackage{slantsc}
\setlength{\parskip}{0.3em}

\DeclareMathOperator*{\argmax}{arg\,max} 

\makeatletter
\newenvironment{algosketch}[1][htb]{%
    \renewcommand{\ALG@name}{Algorithm Sketch}% Update algorithm name
   \begin{algorithm}[#1]%
  }{\end{algorithm}}
\makeatother

\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\declaretheorem[name=Theorem,numberwithin=section]{thm}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{hyp}{Assumption}

\newcommand{\V}{\mathcal{V}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\usepackage{algorithm}
\usepackage{algorithmic}

\newcommand{\SRankElim}{{\sc Pair-Elim}}
\newcommand{\RankElim}{{\sc Rank1Elim}}
\newcommand{\IBLearning}{{\sc Pair-Select}}
\newcommand{\IBLearningname}{Pair Select}
\newcommand{\RMono}{{\sc Pair-Elim-Mono}}
\newcommand{\SMDC}{{\sc simple-Adaptive-Matching}}
\newcommand{\SMDCname}{Simple Adaptive Matching}
\newcommand{\MatchingId}{{\sc Matching-id}}
%\newcommand{\SMDCname}{Simplified Matching Divide and Conquer algorithm}
\newcommand{\MDC}{{\sc Adaptive-Matching}}
\newcommand{\MDCname}{Adaptive Matching}
%\newcommand{\MDCname}{Matching Divide and Conquer}
\newcommand{\CMSampling}{{\sc Sample-Matching}}
\newcommand{\SEBElim}{{\sc Row-Col-Elim}}
\newcommand{\SEBElimR}{{\sc Row-Elim}}
\newcommand{\SEBElimC}{{\sc Col-Elim}}

\newcommand{\fs}[1]{\textcolor{red}{#1}}
\newcommand{\mv}[1]{\textcolor{blue}{#1}}
\newcommand{\jy}[1]{\textcolor{cyan}{#1}}
\newcommand{\cc}[1]{\textcolor{red}{#1}}
\newcommand{\vp}[1]{\textcolor{magenta}{#1}}

\author{%
 
}
